UDON: A case for offloading to general purpose compute on CXL memory

Upcoming CXL-based disaggregated memory devices feature special purpose units to offload compute to near-memory. In this paper, we explore opportunities for offloading compute to general purpose cores on CXL memory devices, thereby enabling a greater utility and diversity of offload. We study two classes of popular memory intensive applications: ML inference and vector database as candidates for computational offload. The study uses Arm AArch64-based dual-socket NUMA systems to emulate CXL type-2 devices. Our study shows promising results. With our ML inference model partitioning strategy for compute offload, we can place up to 90% data in remote memory with just 20% performance trade-off. Offloading Hierarchical Navigable Small World (HNSW) kernels in vector databases can provide upto 6.87$\times$ performance improvement with under 10% offload overhead.

==> acronyms.tex <==
\newacronym{dapc}{DAPC}{Distributed Adaptive Pointer Chasing}
\newacronym{gbpc}{GBPC}{Get-Based Pointer Chasing}
\newacronym{tsi}{TSI}{Target-Side Increment}
\newacronym{xrdma}{X-RDMA}{eXtended Remote Direct Memory Access}
\newacronym{rdma}{RDMA}{Remode Direct Memory Access}
\newacronym{bf2}{BF2}{BlueField-2}

==> design.tex <==
%==============================================================================%
\section{Design and Implementation}
%==============================================================================%



